On the Concurrent Composition of Quantum Zero-Knowledge

We study the notion of zero-knowledge secure against quantum polynomial-time verifiers (referred to as quantum zero-knowledge) in the concurrent composition setting. Despite being extensively studied in the classical setting, concurrent composition in the quantum setting has hardly been studied. We initiate a formal study of concurrent quantum zero-knowledge. Our results are as follows: -Bounded Concurrent QZK for NP and QMA: Assuming post-quantum one-way functions, there exists a quantum zero-knowledge proof system for NP in the bounded concurrent setting. In this setting, we fix a priori the number of verifiers that can simultaneously interact with the prover. Under the same assumption, we also show that there exists a quantum zero-knowledge proof system for QMA in the bounded concurrency setting. -Quantum Proofs of Knowledge: Assuming quantum hardness of learning with errors (QLWE), there exists a bounded concurrent zero-knowledge proof system for NP satisfying quantum proof of knowledge property. Our extraction mechanism simultaneously allows for extraction probability to be negligibly close to acceptance probability (extractability) and also ensures that the prover's state after extraction is statistically close to the prover's state after interacting with the verifier (simulatability). The seminal work of [Unruh EUROCRYPT'12], and all its followups, satisfied a weaker version of extractability property and moreover, did not achieve simulatability. Our result yields a proof of quantum knowledge system for QMA with better parameters than prior works.

==> Temp/coinflip.tex <==
\subsection{Post-Quantum Concurrent Coin-Flipping}
\label{sec:coinflip}
We begin by defining concurrent coin-flipping in the post-quantum setting. Informally, a coin-flipping protocol allows an unbounded party, $P_1$, to interact with a QPT party, $P_2$, in order for both of them to agree and output a random string.
\par To define concurrent coin-flipping formally, we define ${\cal F}$ to be a an input-less two-party functionality that, upon being invoked, outputs a random string to both the parties. We define the security using the simulation paradigm~\cite{Lin17}. 
\par We also define the notion of $Q$-session quantum adversaries below. We define this along the lines of Definition~\ref{def:classical:qadv}.  

\begin{definition}[$Q$-session Quantum  Adversary]
Let $Q \in \mathbb{N}$. Let $\Pi$ be an interactive protocol between a classical PPT algorithm $P_1$ and a classical PPT algorithm $P_2$ for the relation $\rel(\lang)$. Let $(x,w) \in \rel(\lang)$. We say that an adversarial non-uniform QPT verifier $P_2^*$ is a {\bf $Q$-session adversary} if it invokes $Q$ sessions with $P_1$. 
\par Moreover, we assume that the interaction $P_1$ and $P_2^*$ is defined as follows: denote by $P_{2,i}^*$ to be the algorithm used by $P_2^*$ in the $i^{th}$ session and denote by $P_{1,i}$ to be the $i^{th}$ invocation of $P_1$ interacting with $P_{2,i}^*$. Every message sent by $P_2^*$ is of the form $\left( \left(1,\msg_1 \right),\ldots,\left(Q,\msg_Q \right) \right)$, where $\msg_i$ is defined as: 
$$\msg_i = \left\{ \begin{array}{ll} \na, & \text{if }P_{2,i}^*\text{ doesn't send a message},\\ (\rnd,z), & \text{if }P_{2,i}^*\text{ sends }z\text{ in the round }\rnd  \end{array}\right. $$
$P_i$ responds to $\msg_i$. If $\msg_i=\na$ then it sets $\msg'_i=\na$. If $P_{2,i}^*$ has sent the messages in the correct order, then $P_{1,i}$ applies the next message function on its own private state and $\msg_i$ to obtain the quantum state $z'$ and sets $\msg'_i=(t+1,z')$. Otherwise, it sets  $\msg'_i=(\bot,\bot)$. Finally, $P_2^*$ receives $\left( (1,\msg'_1),\ldots,(Q,\msg'_Q) \right)$. %In total, $P_2^*$ exchanges $\ell_{\smprot} \cdot Q$ number of messages, $\ell_{\smprot}$ is the number of the messages in the protocol.
\end{definition}

\noindent Using the notion of $Q$-session quantum adversaries, we define (bounded) concurrent post-quantum coin-flipping protocols below. 

\begin{definition}[(Bounded) Concurrent Post-Quantum Coin-Flipping]
\label{def:pqcoinflip}
Let $Q \in \mathbb{N}$. A protocol $\Pi$, between a classical probabilistic polynomial-time (in $Q$) algorithm $P_1$ and a classical probabilistic polynomial-time (in $Q$) algorithm $P_2$, if the following two conditions are satisfied.
\begin{itemize}
    \item {\bf Completeness}: If both $P_1$ and $P_2$ behave according to the protocol, then the string $r \in \{0,1\}^{\secparam}$ output by both the parties is distributed according to the uniform distribution. 
    \item {\bf Unbounded Simulation Security Against $P_1$}: For every malicious (computationally unbounded) party $P_1^*$, there exists an unbounded simulator $\simulator$ such that such that the output distribution of the honest party along with  $P_1^*$'s output state in the real world is statistically indistinguishable from the output distribution of the honest party along with $P_1^*$'s output state in the ideal world.
    \item {\bf Post-Quantum Simulation Security Against Bounded Concurrent $P_2$}: For every malicious non-uniform $Q$-session adversary $P_2^*$, exists a QPT simulator $\simulator$ such that the output distribution of the honest party along with  $P_2^*$'s output state in the real world is computationally indistinguishable (even against QPT distinguishers) from the output distribution of the honest party along with $P_2^*$'s output state in the ideal world. 
\end{itemize}

\end{definition}

\subsubsection{Construction}
\noindent We start with the template of the quantum-secure instantiation, namely~\cite{damgaard2009quantum},  of Blum's coin-flipping protocol~\cite{blum1983coin}. However,\cite{damgaard2009quantum} uses Watrous rewinding to prove its security. Instead we use a generic zero-knowledge protocol to avoid using Watrous rewinding (at least explicitly). This will also help us achieve concurrent security.   
\par We construct a one-bit coin-flipping protocol. This can be extended to a coin-flipping protocol for long strings by sequential repetition.
\par To construct a bounded concurrent coin-flipping protocol $\Pi$, we use the following ingredients:
\begin{itemize}
    \item Statistical-binding and quantum-concealing commitment scheme, $(\comm,\receiver)$ (see Section~\ref{sec:prelims:commit}).
    \item Bounded concurrent quantum zero-knowledge proof system for the following language, denoted as $\Pi_{\np}$. 
    $$\lang=\left\{ \left((\bfr,\bfc,a)\ ;\ (r) \right)\ :\  \comm(1^{\secparam},\bfr,a;r) = \bfc \right\}$$
    
\end{itemize}
We note that the same construction would yield fully concurrent coin-flipping protocol if one were to start with fully concurrent QZK. 

We describe the construction $\Pi$ in Figure~\ref{fig:ccf}.\\

\begin{figure}[!htb]
   \begin{center}
   \begin{tabular}{|p{16cm}|}
   \hline
    \begin{itemize}
            \item $P_1 \leftrightarrow P_2$: $P_1$ chooses a bit $a \xleftarrow{\$} \{0,1\}$. It then commits to $a$ using the commitment protocol $(\comm,\receiver)$. Let $\bfr$ be the message sent by the receiver and let $\bfc$ be the message sent by the prover. Let $r$ be the randomness used by $P_1$ such that $\comm(1^{\secparam},\bfr,a;r) = \bfc$.
    \item $P_2 \rightarrow P_1$: $P_2$ sends a bit $b \xleftarrow{\$} \{0,1\}$ to $P_1$.
    \item $P_1 \rightarrow P_2$: $P_1$ sends $a$.
    \item $P_1 \leftarrow P_2$: $P_1$ and $P_2$ execute the zero-knowledge protocol, $\Pi_{\np}$, with $P_1$ playing the role of the prover and $P_2$ playing the role of the verifier. The instance is $(\bfr,\bfc,a)$ and the witness is $r$.
    \item Finally, both parties output $s=a\oplus b$.
        
    \end{itemize}
    \\ 
    \hline
   \end{tabular}
    \caption{Construction of Bounded Concurrent Coin-Flipping Protocol.}
    \label{fig:ccf}
    \end{center}
\end{figure}

\noindent We prove the security of $\Pi$ below. 

\begin{lemma}
$\Pi$ is a secure post-quantum coin-flipping bounded-concurrent protocol (Definition~\ref{def:pqcoinflip}). 
\end{lemma}
\begin{proof}
Completeness follows from the completeness of $\Pi_{\np}$. 

\paragraph{Unbounded Simulation Security Against $P_1$.} Suppose $P_1^*$ is a malicious unbounded adversary. 
\par We define a simulator $\simr$ as follows. It receives as input a commitment from $P_1^*$. It then runs in exponential time and finds the bit $a$ committed to by $P_1$. It receives the bit $s$ from the ideal world functionality. It sets $b=s \oplus a$. It sends $b$ to $P_1^*$. It receives $a'$ from $P_1$. If $a' \neq a$ then abort. It then runs the verifier in the ZK protocol $\Pi_{\np}$. 
\par The statistical indistinguishability of the output distributions of the ideal and the real world follow from the statistical binding property of $(\comm,\receiver)$. 

\paragraph{Post-Quantum Simulation Security Against Bounded Concurrent $P_2$.} Suppose $P_2^*$ is a malicious QPT adversary. 
\par We define a simulator $\simr$ as follows. It commits to 0 in the protocol $(\comm,\receiver)$. It receives $b$ from $P_2^*$. It also receives the string $s$ from the ideal world functionality. It computes $a = s \oplus b$. It sends $a$ to $P_2^*$. It then runs the simulator of $\Pi_{\zk}$. 
\par We prove the computational indistinguishability of the output distributions of the ideal and the real world via a hybrid argument. \\

\noindent \underline{$\hybrid_1$}: This corresponds to the real world. \\

\noindent \underline{$\hybrid_2$}: This is the same as the previous hybrid except that the ZK protocol is simulated. 
\par The computational indistinguishability of $\hybrid_1$ and $\hybrid_2$ follows from the quantum zero-knowledge property of $\Pi_{\np}$. \\

\noindent \underline{$\hybrid_3$}: This is the same as the previous hybrid except that the bit committed to in $(\comm,\receiver)$ is 0. 
\par The computational indistinguishability of $\hybrid_2$ and $\hybrid_3$ follows from the computational hiding property of $(\comm,\receiver)$. \\

\noindent \underline{$\hybrid_4$}: This corresponds to the ideal world. 
\par The output distributions of $\hybrid_3$ and $\hybrid_4$ are identical. 

\end{proof}

==> Temp/consQMA.tex <==
\newcommand{\cP}{\mathcal{P}}
\section{Bounded Concurrent QZK for QMA}
We show a construction of bounded concurrent QZK for QMA. Our starting point is the QZK protocol for QMA from \cite{BJSW16}, which constructs QZK for QMA from QZK for NP, commitments and a coin-flipping protocol. We make the following observation about the proof of quantum zero-knowledge in~\cite{BJSW16}. Only two ingredients in their construction require rewinding by the QZK simulator: the coin-flipping protocol and the QZK for NP protocol. The rest of their simulation is straightline -- if we instantiate the coin-flipping protocol and the QZK for NP with ones satisfying (resp., bounded) concurrent security, the resulting QZK for QMA protocol would also satisfy (resp., bounded) concurrent security. We already constructed a bounded concurrent QZK for NP protocol in Section~\ref{sec:BCQZK}. %First we construct a bounded concurrent coin-flipping protocol. Then we will show how to use this to construct a bounded concurrent QZK for QMA. 

\subsection{Bounded Concurrent QZK for QMA}
We first recall the QZK for QMA construction from \cite{BJSW16}. Their protocol is specifically designed for the QMA promise problem called $k$-local Clifford Hamiltonian, which they showed to be QMA-complete for $k = 5$. We restate it here for completeness.

\begin{definition}
[$k$-local Clifford Hamiltonian Problem~\cite{BJSW16}] For all $i \in [m]$, let $H_i = C_i \ket{0^{\otimes k}} \bra{0^{\otimes k}}C^{\dagger}_i$ be a Hamiltonian term on $k$-qubits where $C_i$ is a Clifford circuit. 
\begin{itemize}
    \item Input: $H_1,H_2, \ldots, H_m$ and strings $1^p$, $1^q$ where $p$ and $q$ are positive integers satisfying $2^p > q$.
    \item Yes instances ($A_{yes}$):  There exists an $n$-qubit state such that $\tr[\rho \sum_i H_i]  \leq 2^{-p}$
    \item No instances ($A_{no}$): For every $n$-qubit state $\rho$, the following holds:  $\tr[\rho \sum_i H_i] \geq \frac{1}{q}$
    
\end{itemize}
\end{definition} 

\newcommand{\E}{\mathsf{E}}
\newcommand{\cS}{\mathcal{S}}


\paragraph{BJSW Encoding.} A key idea behind the construction from \cite{BJSW16} is for the prover to encode its witness, $\ket{\psi}$, using a secret-key quantum authentication code (that also serves as an encryption) that satisfies the following key properties needed in the protocol. For any state $\ket{\psi}$, denote the encoding of $\ket{\psi}$ under the secret-key $s$ by $\E_s(\ket{\psi})$. 

\begin{enumerate}

\item {\em Homomorphic evaluation of Cliffords.} Given $\E_s(\ket{\psi})$, and given any Clifford circuit $C$, it is possible to compute $\E_{s'}(C\ket{\psi})$ efficiently. Moreover, $s'$ can be determined efficiently by knowing $C$ and $s$. %\prab{come up $s'$}\\

\item {\em Homomorphic measurements of arbitrary Clifford basis.} For any Clifford circuit $C$ and any state $\ket{\psi}$, a computational basis measurement on $C\ket{\psi}$ can be recovered from a computational basis measurement on $\E_{s'}(C\ket{\psi})$ along with $C$ and $s$. Formally, there is a classically efficiently computable function $g$ such that if $y$ is sampled from the distribution induced by measuring the state $\E_{s'}(C\ket{\psi})$ in the computational basis, then $g(s,C,y)$ is sampled from the distribution induced by measuring the state $C\ket{\psi}$ in the computational basis.

\item {\em Authentication of measurement outcomes.} For any $s$ and any clifford $C$, there is a set $\cS_{s,C}$ such that for any state $\ket{\psi}$, and any computational basis measurement outcome $y$ performed on $\E_{s'}(C \ket{\psi})$, it holds that $y \in \cS_{s,C}$. Furthermore, for any $y$, given $s$ and $C$, it can be efficiently checked whether $y \in \cS_{s,C}$.

\item {\em Simulatability of authenticated states}: there exists an efficient QPT algorithm $B$ such that for any adversary $\adversary$, every $x \in A_{\yes}$ along with witness $\ket{\psi}$, $\poly(\secparam)$-qubit advice $\rho$, the following holds: the probability that $\cP(s,C_{r^*}^{\dagger},\adversary(\E_s(\ket{\psi})))$ outputs 1 is negligibly close to the probability that $\cP(s,C_{r^*}^{\dagger},\adversary(B(x,s,r^*))))$ outputs 1, where $\cP$ is defined below. %We will assume without loss of generality that $B$ outputs a pure state. 
$$\cP(s,C^\dagger,y)=\begin{cases}
1 \text{ if } g(s,C^\dagger,y) \neq 0 \\
0 \text{ otherwise}\end{cases}$$

In both the events, $s$ and $r^*$ are chosen uniformly at random. 

\end{enumerate}



 \noindent The QMA verifier of the $k$-local Clifford Hamiltonian problem measures terms of the form $C \ket{0^{\otimes k}} \bra{0^{\otimes k}}C^\dagger$ where $C$ is a Clifford circuit on a witness $\ket{\psi}$. Specifically, a verifier will first apply $C^\dagger$ and then measure in the computational basis. If the outcome of the measurement is the $0$ string, it rejects.  Otherwise, it accepts.  In the zero-knowledge case, the witness will be encoded, $\E_s(\ket{\psi})$, but the verifier can still compute $\E_{s}(C^\dagger \ket{\psi})$ and measure to obtain some string $y$.  Then, the prover can prove to the verifier (in NP) that $y$ corresponds to a non-zero outcome on a measurement of $C^\dagger \ket{\psi}$ instead using the predicate $\cP$. 


\par We follow the approach of BJSW~\cite{BJSW16}, but we instantiate the underlying primitives with ones satisfying bounded concurrent security. %Following~\cite{coladangelo2020non}, we also add proof of quantum knowledge to the construction.

\paragraph{Construction.} We use the following ingredients in our construction: 
\begin{itemize}
  \item Statistical-binding and quantum-concealing commitment scheme, $(\comm,\receiver)$ ( Section~\ref{sec:prelims:commit}).
   % \item Quantum-secure bounded concurrent QZKPoK system, denoted by $\Pi_{\np}^{(1)}$,  for the following language. 
   % $$\lang^{(1)}=\left\{ \left((\bfr,\bfc,s) ;\ (\ell) \right)\ :\  \comm(1^{\secparam},\bfr,s;\ell) = \bfc \right\}$$
   % \prab{need to get rid of this}
  
  \item Post-quantum bounded-concurrent coin flipping protocol (Section~\ref{sec:coinflip}).
  Let $Q$ be the maximum number of sessions associated with this protocol.
  
  \item Bounded concurrent QZK proof system, denoted by $\Pi_{\np}$, for the following language (Section~\ref{sec:BCQZK}). 
    $$\lang=\left\{ \left((\bfr,\bfc,r^*,y)\ ;\ (s,\ell) \right)\ :\  \left(\cP(s,C_{r^*}^{\dagger},y)=1\right) \bigwedge \comm(1^{\secparam},\bfr,s;\ell) = \bfc \right\}$$
    Let $Q$ be the maximum number of sessions associated with the protocol. 
\end{itemize}

\noindent We describe the construction of bounded concurrent QZK for QMA (with bound $Q$) in Figure~\ref{fig:qmazk}. We prove the following.

%\paragraph{BJSW Protocol.} \ \\

\begin{figure}[!htb]
   \begin{tabular}{|p{16cm}|}
   \hline \\
\par \textbf{Instance:} A $k$-local Clifford Hamiltonian, $H = \overset{M}{\underset{r=1}{\sum}} C_r \ket{0^{\otimes k}} \bra{0^{\otimes k}} C_r^{\dagger}$.
\par \textbf{Witness:} $\ket{\psi}$
\begin{itemize}
    \item $P \leftrightarrow V$: Prover $P$  samples a secret-key $s \xleftarrow{\$} \{0,1\}^{\poly(k,M)}$, and commits to $s$ using the commitment protocol $(\comm,\receiver)$. Let $\bfr$ be the first message of the receiver and $\bfc$ be the commitment.
    \item $P \rightarrow V$: $P$ sends $\E_{s}(\ket{\psi})$.
    \item Prover and verifier perform the coin-flipping protocol $\Pi_{\text{coin}}$ to choose a random element of $\{1,2,...,M\}$. Let $r^*$ be the output.
    \item Verifier computes $\eval \left(C_{r^*}^{\dagger}, \E_{s}(\ket{\Psi})\right) \rightarrow \E_{s}(C_{r^*}^{\dagger} \ket{\psi})$ and measures in the computational basis. Let $y$ denote the measurement outcome. Verifier sends $y$ to the prover.
    \item Prover checks that $y\in \cS_{s,C_{r^*}^{\dagger}}$ and that $\cP(s,C_{r^*}^{\dagger},y)=1$. If not, it aborts. 
    \item Prover and verifier engage in a QZK protocol for $\np$, $\Pi_{\np}$, for the 
    statement $(\bfr,\bfc,r^*,y)$ and the witness $(s,\ell)$. 
  %  following statement:
   % $$\exists (s,\ell) \text{ s.t }  \left(\cP(s,C_{r^*}^{\dagger},y)=1\right) \bigwedge \left( c=\comm(s;\ell)\right) $$
\end{itemize}
\\ 
\hline
\end{tabular}
\label{fig:qmazk}
\caption{Bounded-Concurrent QZK for QMA}
\end{figure}

\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfY}{\mathbf{Y}}
\begin{theorem}
Assuming that $\Pi_{\text{coin}}$ satisfies the definition of post-quantum bounded concurrent coin flipping and $\Pi_{\np}$ satisfies the definition of bounded concurrent QZK for NP, the protocol given in Figure~\ref{fig:qmazk} is a bounded concurrent QZK protocol for $\qma$ with soundness $\frac{1}{\poly}$.
\end{theorem}

\begin{remark}
The soundness of the above protocol can be amplified by sequential repetition. In this case, the prover needs as many copies of the witness as the number of repetitions.
\end{remark}

\begin{proof}[Proof Sketch]
The completeness and soundness follow from~\cite{BJSW16}. We sketch the proof of bounded concurrent zero-knowledge below.

\paragraph{Quantum Zero-Knowledge.} Suppose $x \in A_{\yes}$. Suppose $V^*$ is a non-uniform malicious QPT  $Q$-session verifier. Then we construct a QPT simulator $\simr$ as follows. \\

\noindent \underline{Description of $\simr$}: it starts with the registers $\bfX_{zk},\bfX_{coin},\bfX_{anc},\bfM,\bfY_{ver}$. The register $\bfX_{zk}$ is used by the simulator of the bounded concurrent QZK protocol, $\bfX_{coin}$ is used by the simulator of the bounded concurrent coin flipping protocol, $\bfX_{anc}$ is an ancillary register, $\bfM$ is used to store the messages exchanged between the simulator and the verifier and finally, the register $\bfY_{ver}$ is used for storing the private state of the verifier. Initialize the registers $\bfX_{zk},\bfX_{coin},\bfM$ with all zeroes. Initialize the register $\bfX_{anc}$ with $(\bigotimes_{j=1}^Q\ket{s_j}\bra{s_j}) \otimes (\bigotimes_{j=1}^Q \ket{r^*_j}\bra{r^*_j}) \otimes (\bigotimes_{j=1}^Q \rho_j) \otimes \ket{0^{\otimes \poly}}\bra{0^{\otimes \poly}}$,  where $s_i,r_i^*$ are generated uniformly at random and $\rho_j \leftarrow B(x,s_j,r^*_j)$ is defined in bullet 4 under BJSW encoding. 
\par $\simr$ applies the following unitary for $Q$ times on the above registers. This unitary is defined as follows: it parses the message $((1,\msg_1),\ldots,(Q,\msg_Q))$ in the register $\bfM$. For every round of conversation, it does the following: if it is $V^*$'s turn to talk, it applies $V^*$ on $\bfY_{ver}$ and $\bfM$. Otherwise,  
\begin{itemize}
    \item Let $S_1$ be the set of indices such that for every $i \in S_1$, $\msg_i$ is a message in the protocol $\Pi_{\np}$. Let $S_2$ be the set of indices such that for every $i \in S_2$, $\msg_i$ is a message in the protocol $\Pi_{\text{coin}}$. Finally, let $S_3 = [Q] \backslash (S_1 \cup S_2)$.  
    \item It copies $((1,\msg_1),\ldots,(Q,\msg_Q))$ into $\bfX_{zk}$ (using many CNOT operations) and for every $i \notin S_1$, replaces $\msg_i$ with N/A. It copies $((1,\msg_1),\ldots,(Q,\msg_Q))$ into $\bfX_{\text{coin}}$ and for every $i \notin S_2$, replaces $\msg_i$ with N/A. We note that $\msg_i$ is a quantum state (for instance, it could be a superposition over different messages). 
    
        \item For every $i \in S_3$, if  $\msg_i$ is the first prover's message of the $i^{th}$ session, then set $\msg'_i$ to be $\ket{\bfc_i}\bra{\bfc_i} \otimes \rho_i$, where $\bfc_i$ is the commitment of $s_i$.   
    \item It applies the simulator of $\Pi_{\np}$ on $\bfX_{zk}$ to obtain $ ((1,\msg'_{1,zk}),\ldots(Q,\msg'_{Q,zk}))$. The $i^{th}$ session simulator of $\Pi_{\np}$ takes as input $(\bfr_i,\bfc_i,r^*_i,y_i)$, where $r^*_i$ was generated in the beginning and $\bfr_i,\bfc_i,y_i$ is generated as specified in the protocol. It applies the simulator of $\Pi_{\text{coin}}$ on $\bfX_{coin}$ to obtain $((1,\msg'_{1,coin}),\ldots(Q,\msg'_{Q,coin}))$. The input of the $i^{th}$ session simulator of $\Pi_{\text{coin}}$ is $r^*_i$.
 

    \item Determine $((1,\msg'_1),\ldots,(Q,\msg'_Q))$ as follows. Set $\msg'_i = \msg_{i,\zk}$, if $i \in S_1$. Set $\msg'_i = \msg_{i,coin}$ if $i \in S_2$. Set $\msg'_i = \msg_{i,rest}$ if $i \in S_3$. Output of this round is $((1,\msg'_1),\ldots,(Q,\msg'_Q))$. 
\end{itemize}

\noindent We claim that the output distribution of $\simr$ (ideal world) is computationally indistinguishable from the output distribution of $V^*$ when interacting with the prover (real world). \\

\noindent \underline{$\hybrid_1$}: This corresponds to the real world. \\

\noindent \underline{$\hybrid_2$}: This is the same as $\hybrid_1$ except that the verifier $V^*$ is run in superposition and the transcript is measured at the end. 
\par The output distributions of $\hybrid_1$ and $\hybrid_2$ are identical. \\

\noindent \underline{$\hybrid_{3}$}: Simulate the zero-knowledge protocol $\Pi_{\np}$ simultaneously for all the sessions. Other than this, the rest of the hybrid is the same as before.  
\par The output distributions of $\hybrid_2$ and $\hybrid_3$ are computationally indistinguishable from the bounded concurrent ZK property of $\Pi_{\np}$. \\

\noindent \underline{$\hybrid_4$}: Simulate the coin-flipping protocol $\Pi_{\text{coin}}$ simultaneously for all the sessions. Other than this, the rest of the hybrid is the same as before. 
\par The output distributions of $\hybrid_3$ and $\hybrid_4$ are computationally indistinguishable from the bounded concurrent security of the coin-flipping protocol $\Pi_{\text{coin}}$. \\

\noindent \underline{$\hybrid_{5.i}$ for $i \in [Q]$}: For every $j \leq i$, the commitment in the $j^{th}$ session is a commitment to 0. For all $j > i$, the commitment is computed as in the previous hybrid. 
\par The output distributions of $\hybrid_{5.i-1}$ and $\hybrid_{5.i}$ are computationally indistinguishable from the quantum concealing property of $(\comm,\receiver)$. \\

\noindent \underline{$\hybrid_{6.i}$ for $i \in [Q]$}: For every $j \leq i$, the encoding of the state is computed instead using $B(x,s_i,r^*_i)$, where $s_i,r^*_i$ is generated uniformly at random.
\par The output distributions of $\hybrid_{6.i-1}$ and $\hybrid_{6.i}$ are statistically indistinguishable from simulatability of authenticated states property of BJSW encoding (bullet 4). This follows from the following fact: conditioned on the prover not aborting, the output distributions of the two worlds are identical. Moreover, the property of simulatability of authenticated states shows that the probability of the prover aborting in the previous hybrid is negligibly close to the probability of the prover aborting in this hybrid. \\

\noindent $\underline{\hybrid_7}$: This corresponds to the ideal world. 
\par The output distributions of $\hybrid_{6.Q}$ and $\hybrid_7$ are identical.

\end{proof}

\paragraph{Proof of Quantum Knowledge with better witness quality.} We can define an anologous notion of proof of knowledge in the context of interactive protocols for QMA. This notion is called proof of {\em quantum} knowledge. See~\cite{CVZ20} for a definition of this notion. Coladangelo, Vidick and Zhang~\cite{CVZ20} show how to achieve quantum proof of quantum knowledge generically using quantum proof of classical knowledge. Their protocol builds upon~\cite{BJSW16} to achieve their goal. We can adopt their idea to achieve proof of quantum knowledge property for a bounded concurrent QZK for QMA system. In Figure~\ref{fig:qmazk}, include a quantum proof of classical knowledge system for NP (for instance, the one we constructed in Section~\ref{sec:qzkpok}) just after the prover sends encoding of the witness state $\ket{\Psi}$, encoded using the key $s$. Using the quantum proof of classical knowledge system, the prover convinces the verifier of its knowledge of the $s$. The rest of the protocol is the same as Figure~\ref{fig:qmazk}. 
\par To see why this satisfies proof of quantum knowledge, note that an extractor can extract $s$ with probability negligibly close to the acceptance probability and using $s$, can recover the witness $\ket{\Psi}$. For the first time, we get proof of quantum knowledge (even in the standalone setting) with $1 - \negl$ quality if the acceptance probability is negligibly close to 1, where the quality denotes the closeness to the witness state. Previous proof of quantum knowledge~\cite{BG19,CVZ20} achieved only $1 - \frac{1}{\poly}$ qualtiy; this is because these works use Unruh's quantum proof of classical knowledge technique~\cite{Unruh12} and the extraction probability in Unruh is not negligibly close to the acceptance probability.


==> Temp/oldstuff.tex <==
\section{Obliviousness Conditions}

\begin{definition}[Induced distribution]
Consider two interactive randomized algorithms $A$ and $B$. Let the number of rounds in the protocol between $A$ and $B$ be $t$. 
\par We additionally give the algorithm $A$ the power to rewind the algorithm $B$. We denote $b_{i,j}$ as follows: 
$$b_{i,j} = \left\{ \begin{array}{cl} 0, & \text{A rewinds }i^{th}\text{ round to B's state after }j^{th}\text{ round}\\ 1, & \text{otherwise}  \end{array} \right. $$
\noindent We denote the distribution $\distr$ of $\left( \left\{ b_{i,j} \right\}_{\substack{i > j,}{i,j \ in [t]}} \right)$ and say that $\distr$ is the distribution induced by $(A,B)$. 
\end{definition}

\begin{definition}[Approximate Obliviousness]
Consider a classical zero-knowledge protocol $(P,V)$ for the relation $\rel$ with black-box simulation. 
\par For every malicious verifier $V^*$, there exists a PPT black-box simulator $\simr$ such that the following holds: for every $(x,w) \in \rel$, for every auxiliary information $\aux \in \{0,1\}^{\poly(\secparam)}$, 
$$\left\{ \view_V(\langle P(x,w),V^*(x,\aux) \rangle)  \right\} \approx_c \left\{ \simr^{V^*}(x,\aux) \right\}$$
Suppose $\distr_{\aux}$ be the distribution induced by $(\simr^*(x,\aux),V^*(x,\aux))$. We say that $(P,V)$ satisfies  {\bf $(\varepsilon,\distr)$-approximate obliviousness} condition if there exists a distribution $\distr$ such that the following holds: for every $\aux \in \{0,1\}^{\poly(\secparam)}$,
$$\distr_{\aux} \approx_{s,\varepsilon} \distr$$
\noindent If $\varepsilon$ is negligible, we drop this from the above notation. 
\end{definition}

\begin{definition}[Computational Obliviousness]
Consider a classical zero-knowledge protocol $(P,V)$ for the relation $\rel$ with black-box simulation. 
\par For every malicious verifier $V^*$, there exists a PPT black-box simulator $\simr$ such that the following holds: for every $(x,w) \in \rel$, for every auxiliary information $\aux \in \{0,1\}^{\poly(\secparam)}$, 
$$\left\{ \view_V(\langle P(x,w),V^*(x,\aux) \rangle)  \right\} \approx_c \left\{ \simr^{V^*}(x,\aux) \right\}$$
Suppose $\distr_{\aux}$ be the distribution induced by $(\simr^*(x,\aux),V^*(x,\aux))$. We say that $(P,V)$ satisfies  {\bf $(\varepsilon,\distr)$-computational obliviousness} condition if there exists a distribution $\distr$ such that the following holds: for every $\aux \in \{0,1\}^{\poly(\secparam)}$,
$$\distr_{\aux}\approx_{c,\varepsilon} \distr$$
\noindent If $\varepsilon$ is negligible, we drop this from the above notation. 
\end{definition}

\section{Dream Theorems}

\begin{theorem}[From Obliviousness to Quantum Zero-Knowledge]
\label{thm:olbv:zk}
Let $\distr$ be a distribution on $\{0,1\}^{{t \choose 2}}$. Suppose there exists a $t$-round classical zero-knowledge proof system $(P,V)$ for a language $L$ satisfying $(\varepsilon,\distr)$-computational obliviousness property, where $\varepsilon$ is a negligible function. \par Then, $(P,V)$ satisfies zero-knowledge against quantum polynomial-time verifiers. 
\end{theorem}

\noindent \prab{We need to discuss this - not sure whether we can consider any distribution}

\begin{theorem}[Impossibility of Computational Obliviousness in Concurrent Setting]
\label{thm:comp:oblv}
Suppose there exists a classical (black-box) concurrent zero-knowledge argument system $(P,V)$ for a language $L$ satisfying computational obliviousness property. Then, $L \in BPP$. 
\end{theorem}

\section{From Obliviousness to Quantum Zero-Knowledge}

\subsection{Instantiation: Bounded-Concurrent Zero-Knowledge}

\section{Impossibility of Obliviousness in Concurrent Setting}

\section{Old simulator that didn't work}
The simulator does the following for $i=0 \ldots t$, with $t = Q \cdot \ell$, where $Q$ is the number of verifiers and $\ell$ is the number of messages in any session: 
\begin{itemize} 

\item If $i=0$ (denotes the state before the protocol execution begins): The simulator computes the first round messages of $P$ (prover) in superposition. Let this be in the register $\sfX$, let $\sfY$ contain $\ket{\Psi}$ and finally let $\sfD$ and ?? respectively denote the 1-qubit decision and transcript registers. 

\item For any $i \geq 1$: first the simulator checks if its turn or the verifier's turn; note that all the odd i's correspond to simulator's turn\footnote{Of course multiple verifiers might be trying to communicate with the simulator at the same time. But the simulator after receiving the first message, can block its listening channel and re-open the channel after responding to that message.}. If its the simulator's turn, it does the following: 
\begin{itemize} 
\item Check if its Stage 1 message, if so then execute $P$. 
\item Otherwise, check if ``there exists distinct..." condition in Stage 2 proof is satisfied. If so, use this witness to compute the Stage 2 proof, else abort. 
\end{itemize}
If its the verifier's turn, do the following: 
\begin{itemize} 

\item Check if its a Stage 1 message. 
\par Lets say this message corresponds to $j^{th}$ verifier and the $k^{th}$ slot. If so, check if the corresponding commitment of the simulator is the same as the message bit sent by the $j^{th}$ verifier. If so, set the decision register $\sfD$ to be 0, else set it to be 1. Now, measure this register. If its 0, continue; else apply Watrous rewinding lemma to rewind to the state just after the $(i-1)^{th}$ round message. 
\par If its not a Stage 1 message OR if it is an abort message, sample a bit uniformly at random (\prab{this bit needs to be sampled ahead of time before the protocol execution begins}). Put this bit in $\sfD$. Measure this. If its 0, continue; else apply Watrous rewinding lemma to rewind to the state just after the $(i-1)^{th}$ round message.  
\end{itemize}
{\em NOTE: in either of the two cases, the measurement outcome is $0$ with probability $1/2$.}

\end{itemize}

\section{Simulator claims}
\begin{comment}
\paragraph{Claims to be shown.}

\begin{claim}[Informal]
The unitaries, on which we are applying the Watrous' rewinding lemma, satisfy the obliviousness property.
\end{claim}
\begin{proof}

\end{proof}

\begin{claim}[Informal]
For any $i \in [Q]$, conditioned on the $i^{th}$ verifier not aborting, the probability that the  simulator is able to match at least  $\frac{\ell_{\smslot}}{2} + Q^5 \secparam$ number of commitments is negligibly close to 1. (\prab{not sure probability is the right terminology here})
\end{claim}
\begin{proof}
\prab{need to use the rewinding lemma here.}
\end{proof}

\begin{claim}[Informal]
The transcript along with $\ket{\Psi_{\final}}$ obtained in the ideal experiment is computationally indistinguishable from the transcript along with $\ket{\Psi_{\final}}$ obtained in the real experiment (when interacting with a honest prover). 
\end{claim}
\begin{proof}
\prab{needs to be argued recursively for every block.}
\end{proof}

\end{comment}


==> Temp/temp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Protocol $\Pi$.} Let $s$ be the secret of $P$. Repeat the following for $j=1,\ldots,|s|$.  \par Compute $sh_1,\ldots,sh_{\secparam}$ uniformly at random conditioned on $\oplus_{i=1}^{\secparam} sh_i = s_j$. Repeat the following for $i=1,\ldots,\secparam$ number of times: 

\begin{itemize}
    \item $P$ and $V$ run a statistical OT protocol. $V$ takes the role of the OT receiver with the input of $V$ being $b_i$. $P$ takes the role of the OT sender. It samples a bit $a_i$ uniformly at random and then chooses its input to be $(sh_j,\bot)$ if $a_i=0$, else it chooses its input to be $(\bot,sh_j)$ if $a_i=1$. 
\end{itemize}
At the end of $|s|\secparam$ rounds, $P$ sends $s \oplus w$, where $w$ is the witness of $P$. 

\paragraph{Security.} We consider the following game $G$. This game proceeds as follows: Let $s$ be the secret of $P$. Repeat the following for $j=1,\ldots,|s|$.  \par Compute $sh_1,\ldots,sh_{|s|}$ uniformly at random conditioned on $\oplus_{i=1}^{|s|} sh_i = 0$ ({\bf note the difference from the real experiment}). Repeat the following for $i=1,\ldots,\secparam$ number of times: 

\begin{itemize}
    \item $P$ and $V$ run a statistical OT protocol. $V$ takes the role of the OT receiver with the input of $V$ being $b_i$. $P$ takes the role of the OT sender. It samples a bit $a_i$ uniformly at random and then chooses its input to be $(sh_j,\bot)$ if $a_i=0$, else it chooses its input to be $(\bot,sh_j)$ if $a_i=1$. 
\end{itemize}
At the end of $|s|\secparam$ rounds, $P$ sends $s \oplus w$, where $w$ is the witness of $P$.\\

\noindent We say that security is satisfied if the real experiment and the above ideal experiment is computationally indistinguishable.

\paragraph{Non-uniform advice.} We define an alternate security notion for the protocol $\Pi$. In this notion, the prover $P$ is (non-uniformly) given the randomness $R$ to be used in the protocol and the bits $\{(a_{i,j})\}_{i \in [|s|],j \in [\secparam]}$.  These are defined to be bits such that the probability of the adversary succeeding in the $a_{i,j}^{th}$ OT experiment associated with the $(i,j)^{th}$ execution of OT is negligible (see page 29, \url{https://eprint.iacr.org/2020/235.pdf}). The rest of the security definition is the same as what was defined above; the only difference being that the prover $P$ does not pick $a_i$ uniformly at random in the $j^{th}$ execution. Instead, it uses $a_{i,j}$. 
\par [TO SHOW] if $\Pi$ satisfies the new security notion with non-uniform advice then it also satisfies the above security notion. \prab{this is true if $a_{i,j}$ is a function of only state of verifier and randomness of prover -- the quantum part can be make it messy though since this is not a deterministic function}

\paragraph{Proof of Security for the Non-uniform Advice Setting.} Consider the following hybrids. \\

\noindent \underline{First hybrid}: Real experiment. That is, ignore the $\{a_{i,j}\}$ that were non-uniformly fixed and sample $a_i$ afresh for every $j$. \\ 

\noindent \underline{Second hybrid}: Sample $a'_{i,j}$ afresh. If $\exists i$ such that for every $j$, $a'_{i,j} \neq a_{i,j}$ then abort. 
\par The first and second hybrids are statistically close. This is because: conditioned on the second hybrid not aborting, the distributions are identical. Moreover, the probability that the second hybrid aborts is negligible in $\secparam$. \\

\noindent \underline{Third hybrid}: Sample $a'_{i,j}$ afresh. If $\exists i$ such that for every $j$, $a'_{i,j} \neq a_{i,j}$ then abort. Otherwise, do the following: for every $i$, let $j(i)$ be the index such that $a'_{i,j(i)} = a_{i,j(i)}$. Now, switch the OT sender messages in the $(i,j(i))^{th}$ execution to be $(\bot,\bot)$. 
\par The second and third hybrids are computationally indistinguishable from the security of OT. \\

\noindent \underline{Fourth hybrid}: Share 0 everywhere. 
\par The third and fourth hybrids are identically distributed. \\

\noindent \underline{Fifth hybrid}: put back the shares in every index. 
\par The fourth and fifth hybrids are cmoputationally indistinguishable from the security of OT. \\

\noindent \underline{Sixth hybrid}: Ideal experiment. 
\par The fifth and sixth hybrids are statistically close.

\begin{comment}
\paragraph{Proof.} We focus on the case when $j=1$. We need to argue that there is at least one $i \in \{1,\ldots,\secparam\}rt5$ such that: $a_i \neq $ bit output by the expectation expression in page 29, \url{https://eprint.iacr.org/2020/235.pdf}. Now, we can argue that for this index, $((1-a_i)sh_i + a_i \cdot \bot,(1-a_i)\bot + a_i \cdot sh_i)$ can be switched to $(\bot,\bot)$. We can now argue that the distributions of all the shares of $s_1$ minus the $i^{th}$ one and all the shares of $0$ minus the $i^{th}$ one are identical. 
\end{comment}


